Fundamental Limits of Online Network-Caching

Optimal caching of files in a content distribution network (CDN) is a problem of fundamental and growing commercial interest. Although many different caching algorithms are in use today, the fundamental performance limits of network caching algorithms from an online learning point-of-view remain poorly understood to date. In this paper, we resolve this question in the following two settings: (1) a single user connected to a single cache, and (2) a set of users and a set of caches interconnected through a bipartite network. Recently, an online gradient-based coded caching policy was shown to enjoy sub-linear regret. However, due to the lack of known regret lower bounds, the question of the optimality of the proposed policy was left open. In this paper, we settle this question by deriving tight non-asymptotic regret lower bounds in both of the above settings. In addition to that, we propose a new Follow-the-Perturbed-Leader-based uncoded caching policy with near-optimal regret. Technically, the lower-bounds are obtained by relating the online caching problem to the classic probabilistic paradigm of balls-into-bins. Our proofs make extensive use of a new result on the expected load in the most populated half of the bins, which might also be of independent interest. We evaluate the performance of the caching policies by experimenting with the popular MovieLens dataset and conclude the paper with design recommendations and a list of open problems.

==> Serv_Capacity.tex <==
\section{REGRET ANALYSIS FOR MAXIMUM SERVER CAPACITY CONSTRAINT}

In this section, we will be proving a lower bound on the regret of the online caching when each cache can only serve up to a certain number of users simultaneously. We will be using the usual notations defined in the previous document. We first describe the expression for the reward for a system with a single cache with cache capacity 1 and M users connected to the cache who can each request one of two files at each time step (that is, N=2, C=1). We assume the server capacity is $\alpha$ ($\alpha < M$). We also assume that at every time step, no user is idle, that is, we have M different requests from the users (one per user) at every step. Thus, our algorithm needs to choose which users are to be served at every time step as well as which files are to be cached. The expression for the reward is given by:
\begin{eqnarray}\label{eq:opt_regret}
 & [\sum_{t=1}^T\mathbf{y}_t X_t\mathbf{s}_t] 
\end{eqnarray}
\begin{eqnarray}
\mbox{s.t. $\mathbf{1}_N^T[X_t] \mathbf{s}_t \leq \alpha$ for all t} 
\end{eqnarray}
Here, $\mathbf{s}_t \in [0,1]^N$ is an $N \times 1$ vector which specifies which users are to be served at time step t and $\mathbf{1}_N$ is an $N \times 1$ vector of 1's. $[X_t]$ is a $N \times M$ matrix whose ith column $\mathbf{x}_t^i$ represents the request vector of the ith user at time t. The algorithm chooses $\mathbf{y}_t$ and $\mathbf{s}_t$. Note that elements of $\mathbf{s}_t$ need not be integers. 
We now describe the regret of the algorithm: 
\begin{eqnarray}
\mathbf{y}^*[\sum_{t=1}^T X_t\mathbf{s}_t^*]-[\sum_{t=1}^T\mathbf{y}_t X_t\mathbf{s}_t] 
\end{eqnarray}
\begin{eqnarray}
\mbox{s.t. $\mathbf{1}_N^T[X_t] \mathbf{s}_t^* \leq \alpha$ and $\mathbf{1}_N^T[X_t] \mathbf{s}_t \leq \alpha$ for all t} 
\end{eqnarray}

Here, $\mathbf{y}^*$ is the optimal static caching configuration and $\mathbf{s}_t^*$ is the optimal server policy for time t. The request vectors for each user $\mathbf{x}_t^i$ can be represented as $(q_t^i, 1-q_t^i)$ where $q_t^i$ is a Bernoulli random variable with probability 0.5. Thus, the second term in the regret can be upper bounded using linearity of expectation by $\frac{T\alpha}{2}$ (the general expression is $\frac{CT\alpha}{N}$). Now, we find a lower bound for the first term in the regret. Note that instead of the optimal $s_t^*$, choosing some $s_t$ will give a lower bound for the first term. So we choose $s_t$ as a vector which has 1 in the first $\alpha$ positions and 0 in other positions that is, $s_t=[\underbrace{1,1..,1}_\textrm{$\alpha$ terms},0,0,...]$. This is a valid $s_t$ as upto $\alpha$ requests can be handled at a time. Thus, we get:
\begin{equation}
\begin{split}
   \mathbf{y}^*[\sum_{t=1}^T X_t\mathbf{s}_t^*] &\geq \mathbf{y}^*\sum_{t=1}^T\sum_{i=1}^{\alpha}\mathbf{x}_t^i \\
   &= \mathbf{y}^*(\begin{bmatrix}
           \sum_{t=1}^{T}q_t^1 \\
           T-\sum_{t=1}^{T}q_t^1
         \end{bmatrix}+....+\begin{bmatrix}
           \sum_{t=1}^{T}q_t^{\alpha} \\
           T-\sum_{t=1}^{T}q_t^{\alpha}
         \end{bmatrix}) \\
   &= \mathbf{y}^*(\begin{bmatrix}
           Z_{1} \\
           T-Z_{1}
         \end{bmatrix}+....+\begin{bmatrix}
           Z_{\alpha} \\
           T-Z_{\alpha}
         \end{bmatrix}) \\
    &= \mathbf{y}^*(\begin{bmatrix}
           \sum_{i=1}^{\alpha}Z_i \\
           \alpha T-\sum_{i=1}^{\alpha}Z_i
         \end{bmatrix} \\
    &= max\{\sum_{i=1}^{\alpha}Z_i,\alpha T-\sum_{i=1}^{\alpha}Z_i\}
\end{split}
\end{equation}
We note that $\sum_{i=1}^{\alpha}Z_i$ is a binomial random variable with parameter $(\alpha T,\frac{1}{2})$. Thus, using the previous argument using the mean deviation for the binomial distribution, we can get the lower bound on expected value of this term:
\begin{equation}
    \mathrm{E}[\mathbf{y}^*[\sum_{t=1}^T X_t\mathbf{s}_t^*]] \geq \frac{\alpha T}{2}+O(\sqrt{\alpha T})
\end{equation}
Thus,we get a lower bound of $O(\sqrt{T})$ on the regret for this case.

We can easily apply this argument for the general case of N files using the ``balls into bins'' argument used previously by recursively grouping the bins into 2 superbins at each stage (for log N stages). We can also extend this argument for general cache capacity C by grouping the bins into $\frac{N}{C}$ superbins as was done previously. Finally, this analysis can be extended for the most general case with $J$ caches each having a cache capacity of $C_j$, by simply lower bounding the optimal utility for each cache independently and then summing them up (that is, lower bounding $\sum_{j=1}^{J}{\mathbf{y}^j}^*[\sum_{t=1}^T X_t{\mathbf{s}_t^j}^*]$). While finding the lower bound for each cache,we can choose $\mathbf{s}_t^j$ as a vector with 1 in first $\alpha_j$ positions and 0's elsewhere.

%\newpage

==> acknowledgement.tex <==
\section{Acknowledgement}
This work is supported by the Qualcomm grant IND-417880. The last author would like to thank Georgios Paschos for introducing him to the online caching problem.
